The Development of the NNBAR Experiment

The NNBAR experiment for the European Spallation Source will search for free neutrons converting to antineutrons with a sensitivity improvement of three orders of magnitude compared to the last such search. This paper describes progress towards a conceptual design report for NNBAR. The design of a moderator, neutron reflector, beamline, shielding and annihilation detector is reported. The simulations used form part of a model which will be used for optimisation of the experiment design and quantification of its sensitivity.

==> simulationframework.tex <==
\section{A simulation model for the NNBAR experiment}
\label{sec:simulationframework}
% actually we could mention the full, but summarized framework that is in: https://arxiv.org/abs/2106.15898 - but in such case it would be better to have it in a separate section and not within detector

\subsubsection{The simulation chain}  
\label{sec:chain} 
 
To quantify the sensitivity of the  $n\rightarrow\bar{n}$ search, the full design of the experiment has to be carried out. This includes the design of the ESS lower moderator, the beam extraction system that exploits the large beam port, the field-free propagation region and beamline, and finally the design of a detector able to observe an annihilation signal. 
In order to do this a connected chain of different simulation programs is required~\cite{Meirose2021}. 

\begin{figure*}[ht]
    \centering
    \includegraphics[height=5.75cm]{images/SImulationChainFinal.png}
    \caption{Top: A schematic view of the different components needed for the NNBAR experiment. Bottom: a simulation flowchart; the moderator is simulated and optimized with \software{MCNP6}. All \software{MCNP6} simulation results are passed to \software{McStas} with \software{MCPL} and then as last stage of the simulation they are passed to \software{GEANT4} for the simulation of the detector. Adapted from Ref.~\cite{Meirose2021}.   %The reflector simulations is performed with the that will provide the neutronics
    }
    \label{fig:simchain}
\end{figure*}

The neutrons that are produced by ESS can be divided into two main categories: (i) cold neutrons (with energies below \textless 1eV) (ii) fast neutrons (with energies above \textgreater 1eV). The cold neutrons, those that are used for the NNBAR experiment and the neutron scattering instruments,  are studied and simulated with ray-tracing codes such \software{McStas}~\cite{willendrup2004_McStasNew}
while neutrons with higher energies, that may provide background to NNBAR, require radiation transport code such as \software{MCNP} \cite{ref_MCNP6} or \software{PHITS}~\cite{phits}. The NNBAR detector is simulated with \software{GEANT4}~\cite{Agostinelli:2002hh},  a standard simulation package used for detector simulations.


To make it possible for all these programs to exchange the data produced by each simulation the \software{MCPL}~\cite{KITTELMANN201717} package is used, which is a binary format storing information on the state of a particle (momentum and position) and allows for interchanging of trajectories, particles, or entire events over different Monte Carlo-based simulation programs. Figure~\ref{fig:simchain} gives an overview of the simulation chain that has been used to construct the full model of the NNBAR experiment. It comprises a number of components, each representing distinct aspects of the experiment and effectively follows the neutron as it is focused and propagates towards the annihilation detector. The simulation of the neutron source must first be done. The reflection and focusing of neutrons is then modelled prior to the simulation of propagation of neutrons in a suppressed magnetic field region (also studied and optmized in the chain using the  finite-element simulations tool \software{COMSOL}~\cite{multiphysics1998introduction}) in a vacuum tube towards a carbon foil target on which antineutrons would annihilate giving rise to an isotropic multi-pion final state.
The annihilation events are simulated with  a generator that assumes an initial antineutron impinging on a carbon nucleus~\citep{Golubeva:2018mrz,Barrow:2019viz,Barrow:2021odz}; the annihilation occurs predominately at the surface of the nucleus, and the generator then provides predictions of final state particle four momenta and particle identities in a proprietary format. A translation of this format into a structure legible by \software{MCPL}, which is then integrated into the final \software{GEANT4} simulation of the annihilation detector.
%which observes $\bar{n}N$ annihilations\footnote{The letters $A$ and $N$ are used in this work to denote a nucleus and a nucleon, respectively.} must then be modelled. 
Interactions of backgrounds (e.g. fast spallation products) with the foil must also be simulated. External backgrounds, e.g. due to cosmic rays, are also required. The energy and tracking reconstruction software has been developed by HIBEAM/NNBAR collaboration. 

%MCPL is a binary format which lists particle state (neutron trajectory) information and allows for interchanging of trajectories, particles, or entire events across various Monte Carlo simulation applications



